Hybrid divide-and-conquer approach for tree search algorithms

One of the challenges of quantum computers in the near- and mid- term is the limited number of qubits we can use for computations. Finding methods that achieve useful quantum improvements under size limitations is thus a key question in the field. In this vein, it was recently shown that a hybrid classical-quantum method can help provide polynomial speed-ups to classical divide-and-conquer algorithms, even when only given access to a quantum computer much smaller than the problem itself. In this work, we study the hybrid divide-and-conquer method in the context of tree search algorithms, and extend it by including quantum backtracking, which allows better results than previous Grover-based methods. Further, we provide general criteria for polynomial speed-ups in the tree search context, and provide a number of examples where polynomial speed ups, using arbitrarily smaller quantum computers, can be obtained. We provide conditions for speedups for the well known algorithm of DPLL, and we prove threshold-free speed-ups for the PPSZ algorithm (the core of the fastest exact Boolean satisfiability solver) for well-behaved classes of formulas. We also provide a simple example where speed-ups can be obtained in an algorithm-independent fashion, under certain well-studied complexity-theoretical assumptions. Finally, we briefly discuss the fundamental limitations of hybrid methods in providing speed-ups for larger problems.

==> qpic/siar.tex <==
\begin{tikzpicture}[scale=1.000000,x=1pt,y=1pt]
\filldraw[color=white] (0.000000, -7.500000) rectangle (316.000000, 112.500000);
% Drawing wires
% Line 1: a W M_{-1} \cdots
\draw[color=black] (0.000000,105.000000) -- (26.000000,105.000000);
\draw[color=black] (26.000000,105.000000) -- (33.500000,105.000000);
\draw[color=black] (33.500000,105.000000) -- (41.000000,105.000000);
\draw[color=black] (41.000000,105.000000) -- (100.000000,105.000000);
\draw[color=black] (100.000000,105.000000) -- (107.500000,105.000000);
\draw[color=black] (107.500000,105.000000) -- (115.000000,105.000000);
\draw[color=black] (115.000000,105.000000) -- (174.000000,105.000000);
\draw[color=black] (174.000000,105.000000) -- (181.500000,105.000000);
\draw[color=black] (181.500000,105.000000) -- (189.000000,105.000000);
\draw[color=black] (189.000000,105.000000) -- (248.000000,105.000000);
\draw[color=black] (248.000000,105.000000) -- (255.500000,105.000000);
\draw[color=black] (255.500000,105.000000) -- (263.000000,105.000000);
\draw[color=black] (263.000000,105.000000) -- (316.000000,105.000000);
\draw[color=black] (0.000000,105.000000) node[left] {$M_{-1}$};
% Line 2: b W M_0 \cdots
\draw[color=black] (0.000000,90.000000) -- (26.000000,90.000000);
\draw[color=black] (26.000000,90.000000) -- (33.500000,90.000000);
\draw[color=black] (33.500000,90.000000) -- (41.000000,90.000000);
\draw[color=black] (41.000000,90.000000) -- (100.000000,90.000000);
\draw[color=black] (100.000000,90.000000) -- (107.500000,90.000000);
\draw[color=black] (107.500000,90.000000) -- (115.000000,90.000000);
\draw[color=black] (115.000000,90.000000) -- (174.000000,90.000000);
\draw[color=black] (174.000000,90.000000) -- (181.500000,90.000000);
\draw[color=black] (181.500000,90.000000) -- (189.000000,90.000000);
\draw[color=black] (189.000000,90.000000) -- (248.000000,90.000000);
\draw[color=black] (248.000000,90.000000) -- (255.500000,90.000000);
\draw[color=black] (255.500000,90.000000) -- (263.000000,90.000000);
\draw[color=black] (263.000000,90.000000) -- (316.000000,90.000000);
\draw[color=black] (0.000000,90.000000) node[left] {$M_0$};
% Line 3: c W M_1 \cdots
\draw[color=black,rounded corners=4.000000pt] (0.000000,75.000000) -- (26.000000,75.000000) -- (33.500000,67.500000);
\draw[color=black,rounded corners=4.000000pt] (33.500000,67.500000) -- (41.000000,60.000000) -- (100.000000,60.000000) -- (107.500000,67.500000);
\draw[color=black,rounded corners=4.000000pt] (107.500000,67.500000) -- (115.000000,75.000000) -- (174.000000,75.000000) -- (181.500000,67.500000);
\draw[color=black,rounded corners=4.000000pt] (181.500000,67.500000) -- (189.000000,60.000000) -- (248.000000,60.000000) -- (255.500000,67.500000);
\draw[color=black,rounded corners=4.000000pt] (255.500000,67.500000) -- (263.000000,75.000000) -- (316.000000,75.000000);
\draw[color=black] (0.000000,75.000000) node[left] {$M_1$};
% Line 4: d W M_2 \cdots
\draw[color=black,rounded corners=4.000000pt] (0.000000,60.000000) -- (26.000000,60.000000) -- (33.500000,45.000000);
\draw[color=black,rounded corners=4.000000pt] (33.500000,45.000000) -- (41.000000,30.000000) -- (100.000000,30.000000);
\draw[color=black] (100.000000,30.000000) -- (107.500000,30.000000);
\draw[color=black] (107.500000,30.000000) -- (115.000000,30.000000);
\draw[color=black] (115.000000,30.000000) -- (174.000000,30.000000);
\draw[color=black] (174.000000,30.000000) -- (181.500000,30.000000);
\draw[color=black] (181.500000,30.000000) -- (189.000000,30.000000);
\draw[color=black,rounded corners=4.000000pt] (189.000000,30.000000) -- (248.000000,30.000000) -- (255.500000,45.000000);
\draw[color=black,rounded corners=4.000000pt] (255.500000,45.000000) -- (263.000000,60.000000) -- (316.000000,60.000000);
\draw[color=black] (0.000000,60.000000) node[left] {$M_2$};
% Line 5: ...e W
\draw[color=black] (0.000000,45.000000) node[anchor=mid east] {$\vdots$};
% Line 6: f W M_{k-1} \cdots
\draw[color=black,rounded corners=4.000000pt] (0.000000,30.000000) -- (26.000000,30.000000) -- (33.500000,22.500000);
\draw[color=black,rounded corners=4.000000pt] (33.500000,22.500000) -- (41.000000,15.000000) -- (100.000000,15.000000);
\draw[color=black] (100.000000,15.000000) -- (107.500000,15.000000);
\draw[color=black] (107.500000,15.000000) -- (115.000000,15.000000);
\draw[color=black] (115.000000,15.000000) -- (174.000000,15.000000);
\draw[color=black] (174.000000,15.000000) -- (181.500000,15.000000);
\draw[color=black] (181.500000,15.000000) -- (189.000000,15.000000);
\draw[color=black] (189.000000,15.000000) -- (248.000000,15.000000);
\draw[color=black] (248.000000,15.000000) -- (255.500000,15.000000);
\draw[color=black] (255.500000,15.000000) -- (263.000000,15.000000);
\draw[color=black] (263.000000,15.000000) -- (316.000000,15.000000);
\draw[color=black] (0.000000,30.000000) node[left] {$M_{k-1}$};
% Line 7: g W M_k \cdots
\draw[color=black,rounded corners=4.000000pt] (0.000000,15.000000) -- (26.000000,15.000000) -- (33.500000,7.500000);
\draw[color=black,rounded corners=4.000000pt] (33.500000,7.500000) -- (41.000000,0.000000) -- (100.000000,0.000000);
\draw[color=black] (100.000000,0.000000) -- (107.500000,0.000000);
\draw[color=black] (107.500000,0.000000) -- (115.000000,0.000000);
\draw[color=black] (115.000000,0.000000) -- (174.000000,0.000000);
\draw[color=black] (174.000000,0.000000) -- (181.500000,0.000000);
\draw[color=black] (181.500000,0.000000) -- (189.000000,0.000000);
\draw[color=black] (189.000000,0.000000) -- (248.000000,0.000000);
\draw[color=black] (248.000000,0.000000) -- (255.500000,0.000000);
\draw[color=black] (255.500000,0.000000) -- (263.000000,0.000000);
\draw[color=black] (263.000000,0.000000) -- (316.000000,0.000000);
\draw[color=black] (0.000000,15.000000) node[left] {$M_k$};
% Line 8: h W a_b color=blue \cdots
\draw[color=blue,rounded corners=4.000000pt] (0.000000,0.000000) -- (26.000000,0.000000) -- (33.500000,37.500000);
\draw[color=blue,rounded corners=4.000000pt] (33.500000,37.500000) -- (41.000000,75.000000) -- (100.000000,75.000000) -- (107.500000,67.500000);
\draw[color=blue,rounded corners=4.000000pt] (107.500000,67.500000) -- (115.000000,60.000000) -- (174.000000,60.000000) -- (181.500000,67.500000);
\draw[color=blue,rounded corners=4.000000pt] (181.500000,67.500000) -- (189.000000,75.000000) -- (248.000000,75.000000) -- (255.500000,52.500000);
\draw[color=blue,rounded corners=4.000000pt] (255.500000,52.500000) -- (263.000000,30.000000) -- (316.000000,30.000000);
\draw[color=blue] (0.000000,0.000000) node[left] {$a_b$};
% Done with wires; drawing gates
% Line 9: a /
\draw (6.000000, 99.000000) -- (14.000000, 111.000000);
% Line 10: b /
\draw (6.000000, 84.000000) -- (14.000000, 96.000000);
% Line 11: c /
\draw (6.000000, 69.000000) -- (14.000000, 81.000000);
% Line 12: d /
\draw (6.000000, 54.000000) -- (14.000000, 66.000000);
% Line 13: f /
\draw (6.000000, 24.000000) -- (14.000000, 36.000000);
% Line 14: g /
\draw (6.000000, 9.000000) -- (14.000000, 21.000000);
% Line 15: h /
\draw (6.000000, -6.000000) -- (14.000000, 6.000000);
% Line 16: a b h c d f g PERMUTE
% Line 17: a b h G $\text{SIAB}_1$ width=35
\draw (70.500000,105.000000) -- (70.500000,75.000000);
\begin{scope}
\draw[fill=white] (70.500000, 90.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\clip (70.500000, 90.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\draw (70.500000, 90.000000) node {$\text{SIAB}_1$};
\end{scope}
% Line 18: a b c h d f g PERMUTE
% Line 19: b c h G $\text{SIAB}_2$ width=35
\draw (144.500000,90.000000) -- (144.500000,60.000000);
\begin{scope}
\draw[fill=white] (144.500000, 75.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\clip (144.500000, 75.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\draw (144.500000, 75.000000) node {$\text{SIAB}_2$};
\end{scope}
% Line 20: a b h c d f g PERMUTE
% Line 21: a b h G $\text{SIAB}_1$ width=35
\draw (218.500000,105.000000) -- (218.500000,75.000000);
\begin{scope}
\draw[fill=white] (218.500000, 90.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\clip (218.500000, 90.000000) +(-45.000000:24.748737pt and 29.698485pt) -- +(45.000000:24.748737pt and 29.698485pt) -- +(135.000000:24.748737pt and 29.698485pt) -- +(225.000000:24.748737pt and 29.698485pt) -- cycle;
\draw (218.500000, 90.000000) node {$\text{SIAB}_1$};
\end{scope}
% Line 22: a b c d h f g PERMUTE
% Line 23: c d h G $\text{SIAB}_3$ width=35
\draw (292.500000,75.000000) -- (292.500000,30.000000);
\begin{scope}
\draw[fill=white] (292.500000, 52.500000) +(-45.000000:24.748737pt and 40.305087pt) -- +(45.000000:24.748737pt and 40.305087pt) -- +(135.000000:24.748737pt and 40.305087pt) -- +(225.000000:24.748737pt and 40.305087pt) -- cycle;
\clip (292.500000, 52.500000) +(-45.000000:24.748737pt and 40.305087pt) -- +(45.000000:24.748737pt and 40.305087pt) -- +(135.000000:24.748737pt and 40.305087pt) -- +(225.000000:24.748737pt and 40.305087pt) -- cycle;
\draw (292.500000, 52.500000) node {$\text{SIAB}_3$};
\end{scope}
% Done with gates; drawing ending labels
\draw[color=black] (316.000000,105.000000) node[right] {$\cdots$};
\draw[color=black] (316.000000,90.000000) node[right] {$\cdots$};
\draw[color=black] (316.000000,75.000000) node[right] {$\cdots$};
\draw[color=black] (316.000000,60.000000) node[right] {$\cdots$};
\draw[color=black] (316.000000,45.000000) node[anchor=mid west] {$\vdots$};
\draw[color=black] (316.000000,15.000000) node[right] {$\cdots$};
\draw[color=black] (316.000000,0.000000) node[right] {$\cdots$};
\draw[color=blue] (316.000000,30.000000) node[right] {$\cdots$};
% Done with ending labels; drawing cut lines and comments
% Done with comments
\end{tikzpicture}


==> rev-s-sia.tex <==
\defmath\as{|\vec{a}_{s}|}
\defmath\ssiar{S_{\mathit{r}}}
\defmath\tsiar{T_{\mathit{r}}}
\defmath\ssia{S_{\mathit{b}}}
\defmath\tsia{T_{\mathit{b}}}

\defmath\ssias{S_{\mathit{s}}}
\defmath\tsias{T_{\mathit{s}}}

\defmath\ks{{k_{s}}}
\defmath\kr{{k_{r}}}

\defmath\lolo{\mathrm{ll}}

In this section, we realize a reversible implementation of $s$-implication-with-advice ($s$-SIA) for a $w$-bounded index width ($w$-biw) formula $F$ using a pebbling strategy due to Bennett~\cite{bennett}, which allows for a spacially efficient implementation. 
We define $s$-implication-with-advice ($s$-SIA) to be Algorithm~\ref{algorithm:meta-rez} with $s$-implication as reduction rule.

The degree $d$ of Boolean formulas $F$, which is defined to be the upper bound of the number of clauses in which a variable appears, is unrestricted.

\begin{theorem}\label{t:main}
There is a reversible circuit that computes $s$-SIA for a $w$-bounded index width ($w$-biw) formula $F$ with $n$ variables using  
 $T(n) \in O(3^{\log(\nicefrac nw)} \cdot w \cdot  d^s \cdot \lolo(n))$ 
 time and 
 $S(n) \in O(w \cdot \log^2(\nicefrac nw) + \log(n))$
 space (wires),
 where $\lolo(n) = \log\log(n)$.
\end{theorem} 

The remainder of this appendix is dedicated to a proof of this theorem. We adopt the following strategy: we split the SIA computation in blocks of size $w$. There are $\zeta = n / w$ blocks 
(assuming $w$ divides $n$): each block assigns $w$ variables of the function $F$ according to the specification of $s$-implication-with-advice ($s$-SIA) and increments a pointer $\vec p$ to the next unused advice index.

In what follows, indices start from~$1$, and ranges are manipulated algebraically, e.g, $3 + [1..x] = [4..x+3]$. We take circuit depth as a measure of time. 

For a block $1 \le i \le \zeta$, the type of the function computing it is:
\[
o_1, ..., o_w, \vec p, r, \vec a_{b}  :=  SIAB_i (i_1, ..., i_w, \vec  p, r, \vec a_{b})
\]
where the function $SIAB_i$ computes the values (outputs $\vec o$) for variables of $F$ indexed $i \cdot w + [1 .. w]$, based on the inputs $(i-1) \cdot w + [1 .. w]$, unless input $r$ (a flag) is set, in which case it is the identity function. 

%Note that those are logical, not physical, inputs and outputs. 
The variable $r$ is flag implemented as a counter, which we also provide as input to the SIAB function (just like $\vec p$), in order to make the function recursively composable.

Moreover, if the function $SIAB_i$ encounters a contradiction or runs out of advice, it sets the flag $r$ up. The additional ancillas it requires are provided as $\vec a_{b}$.

We omit the advice memory tape from the parameters as it is read-only in the specification of SIAB.
We denote the size of inputs / outputs as
$S = |\vec i| + \sizeof{\vec p} + \sizeof r = |\vec o| + \sizeof{\vec p} + \sizeof r \in O(w + \log(n))$.

Note that $SIAB_1$ computes the initialization of the procedure for $\vec p = r = 0$,
no matter $\vec i$.

The composition $SIAC = SIAB_l \circ ... \circ SIAB_1$ now computes the value we are interested in. Note that for a given advice, this clearly is a deterministic computation ($SIAB_i$ is a function). The computation is however not reversible, since the function is not a bijection.


While SIA can be implemented and used reversibly at low cost, our implementation of SIAC is more involved.

\begin{lemma}\label{l:sia}
$SIAB_i$ can be implemented reversibly in  $\tsia \in O(w \cdot d^s \cdot \lolo(n))$ time and
$\ssia \in  O(w + \log(n))= S$ space (including $O(\log(n))$ for ancillas $a_b$),
where ``reversibly'' means that, the ancillas $\vec a_{b}$ are always restored to their value prior to the SIAB call and the output can be uncomputed by calling SIAB again (SIAB is its own inverse).
\end{lemma}

\begin{proof}
We implement $SIAB_i$ reversibly by applying the identity to the input wires and ancillas, and XOR to the output wires. We introduce the following notation, where variables are on separate wires, in order to make function composition easier:
\[
o_1, ..., o_w, \vec p', r'  \xor  SIAB_i (i_1, ..., i_w,  \vec  p, r, \vec a_b)
\]

A procedure which involves the deletion of variables arguably constitute an obstacle towards reversibility. We can avoid this obstacle by keeping values for $2\cdot w$ variables on input and output wires.

In time $d^s$, we iterate over all $s$-sized subformulae,
using counters of $a_b =\log(n)$ additional ancillas, thus taking $\lolo(n) = \log(\log(n))$ time to update.
Because we have all $2w$ variables, it is trivial to uncompute ancillas.
\end{proof}

\begin{remark}
To make $SIAC$ reversible similarly, 
we need to copy SIAB input/outputs $\zeta$ times plus the (reusable) ancillas for SIAB,
thus requiring $|a_r| = \zeta\cdot S + |a_b|$ ancillas. \hfill$\blacktriangleleft$ 
\end{remark}

Now we turn our attention to making SIAC reversible with fewer wires $\ssiar = S + |a_r|$
and reasonable time \tsiar. For a given advice, view this function composition as a line graph. The intermediary nodes in the graph represent the intermediary states of only
inputs/outputs, i.e., $S$ bits, and the graph has $\zeta$ such nodes. Note that ancillas are thus not part of the intermediary states, as they are restored to their original value (0) and can be reused.

The reversible procedure developed here is based on games played on directed graphs, called the reversible pebble games. The rules of such reversible pebble game can be defined as follows: one can (un)pebbled the first node (on the line) for free, whereas any other node can only be (un)pebbled once its predecessor is pebbled; one wins the game if one can put a pebble on the target node.

A pebbling configuration is a set of pebbled graph nodes. A pebbling strategy is a sequence of pebbling configurations, where consecutive pairs of configurations adhere to the rules of the game. A strategy
should also end with a configuration containing only the last node of the graph,
so that all intermediate results are uncomputed (unpebbled) and the computation is reversible by executing it
again (reverting the last node by unpebbling).

A trivial strategy lays a pebble on all nodes sequentially. Such a strategy is easy to uncompute by reversing the order, as all nodes have their predecessors pebbled. 
This is equivalent to copying the wires $\zeta$ times as illustrated above, thus will yield 
$\sizeof{a_r} = (\zeta-1)\cdot S + |a_b| = O(\zeta(w+\log(n))) = O(n+\zeta\cdot\log(n))$ ancillas for
the reversible SIA procedure (but we were aiming for a $o(n)$).

In general (as we will show), if there exists a strategy with $p$ pebbles, the computation of SIAC can be simulated reversibly using only $\ssiar = |a_s| = O(p\cdot S + |a_b|)$ space. Moreover, if we can explicitly construct a strategy (sequence of configurations) of length $e$, then the reversible simulation can be carried out in $e \cdot T_b$ time.
Taking the naive approach with $e=\zeta$ pebbles,
we obtain $T_r = 2 \zeta \cdot T_b$, i.e., the same as the irreversible time of SIAC.

Bennett's algorithm (which implements a concrete pebbling strategy \cite{bennett}) is such that a line graph of length $\zeta$ can be (reversibly) pebbled with only $p = \log(\zeta)$ pebbles. This follows from a simple inductive argument: To (un)pebble the last node $c$ on the line graph $a .. c$ with $a=1$ and $c=\zeta$ using $p=\log(\zeta)$ pebbles, we can first pebble the midpoint $b = \zeta/2$ with $p-1$ pebbles, then pebble $b..c$  with $p-1$ pebbles, before unpebbling $b$ with $p-1$ pebbles, in each case applying the induction hypothesis. In the base case, we need $p=log(1)=0$ pebbles to compute a single step in the graph as no intermediate results have to be stored. 

We show that this induction hypothesis can be strengthened to include the reversibility of the pebbles, i.e., that the ancillas storing sub-problems results (pebbles) are restored to their original value.

\begin{figure}
\mbox{
 \Qcircuit @C=1em @R=1em {
  \lstick{M_{-1}} & {/} \qw &  \multigate{1}{\texttt{SIAB}_1}  & \qw & \multigate{1}{\texttt{SIAB}_1} & \qw & \qw & \rstick{\cdots} \\
  \lstick{M_0} & {/} \qw & \ghost{\texttt{SIAB}_1} & \multigate{1}{\texttt{SIAB}_2} & \ghost{\texttt{SIAB}_1} & \qw & \qw & \rstick{\cdots} \\
  \lstick{M_1} & {/} \qw & \qw & \ghost{\texttt{SIAB}_2} & \qw & \multigate{1}{\texttt{SIAB}_3} & \qw & \rstick{\cdots} \\
  \lstick{M_2} & {/} \qw & \qw & \qw & \qw & \ghost{\texttt{SIAB}_3} & \qw & \rstick{\cdots}\\
  & & \vdots & & \vdots & & \vdots \\
  \ \\
  \lstick{M_k} & {/} \qw & \qw & \qw & \qw & \qw & \qw  & \rstick{\cdots}\\
  \ \\
  \lstick{a_b} & {/} \qw & \qw & \qw & \qw & \qw & \qw & \rstick{\cdots}
 }
 }
\caption{\label{fig:siar} Circuit for SIAR}
\end{figure}

We define SIAR (see Figure~\ref{fig:siar} for a representation and Figure~\ref{algorithm:siar} for a pseudocode), which computes SIA reversibly using (1) Bennett's pebbling strategy, (2) the  $SIAB_i$ blocks and (3) $k= \log(\zeta)$ pebbles.
%Bennett splits the line-graph into $2^k$ segments of size $m = \zeta / 2^k$ for $0 \le k \le log(\zeta)$. Hence, by the above argument, the segments can be pebbled with $\log(2^k) = k$ pebbles.
SIAR has the same $S$ input and output wires as SIAC/SIAB, denoted here as
$M[-1]$ and $M[k]$.
The ancillas it uses consist of the $k$
pebbles storing intermediate results,
denoted as array of $S$-sized memory cells $M[0 .. k-1]$,
plus ancillas of SIAB.
So $a_r=k \cdot S + |a_b|$.
Ancillas $a_r$ are reset and SIAR is its own reverse,
so $M[k]$ is restored to zero by calling it again. Note that this facilitates the strengthening of the induction hypothesis.


The parameters $a$ and $c$ (derived) indicate the sequence of SIAB blocks that is computed.
Similar to the inductive argument above, the algorithm splits the sequence $a .. c$ by taking its
exact midpoint $b$.
The parameters $s,t$ control which of the pebbles contain the input and output values of the 
operation, i.e, from $M[s]$ to $M[t]$, while $p$ stipulates how many pebbles can be used for intermediate results (reversibly, i.e., their original values should be restored).
They ensure that the $k$ pebbles are reused succinctly during the computation, as illustrated in Figure~\ref{fig:trees1} and Figure~\ref{fig:trees2}.
The third of the three recursive calls takes care of reversing intermediate results.

\begin{figure*}
\centering
%\lstset{basicstyle=\footnotesize}
\begin{lstlisting}
SIAR(1, -1, k, k)  (*$\hfill\blacktriangleleft$\textrm{Initial call: compute blocks $1$ .. $2^k$ from pebble $-1$ into $k$ using $k$ pebbles}*) (*\vspace{.3em}*)
SIAR(a, s, t, p)    (*$\hfill\blacktriangleleft$\textrm{compute blocks $a$ .. $c$ with $c = s+2^p$ using $p$ pebbles: 0 .. $p-1$}*)
    if (p = 0)
        M[t]$ \xor SIAB_{a}$(M[s], $a_b$) (*$\hfill\blacktriangleleft$  \textrm{compute the blocks $a$ .. $a+1$ from pebble s into t}*)
    else
        r := p - 1   (*$\hfill\blacktriangleleft$ \textrm{r is the midway pebble}*)
        b := $\mathsf a + 2^{\mathsf r}$   (*$\hfill\blacktriangleleft$ \textrm{b is midway between blocks a .. c}*)
        SIAR(a, s, r, p-1) (*$\hfill\blacktriangleleft$ \textrm{compute blocks a .. b using pebbles p-2 .. 0}*)
        SIAR(b, r, t, p-1) (*$\hfill\blacktriangleleft$ \textrm{compute blocks b .. c using pebbles p-2 .. 0}*)
        SIAR(a, s, r, p-1)   (*$\hfill\blacktriangleleft$ \textrm{uncompute blocks a .. b using pebbles p-2 .. 0}*)(*\vspace{-.2em}*) 
\end{lstlisting}
\caption{SIAR}
\label{algorithm:siar}
\end{figure*}

\begin{figure*}
\begin{forest}
for tree={draw, l sep=15pt},
before drawing tree={
    tikz+={
      \node [anchor=mid east] (m) at (current bounding box.west |- .mid) {p=3};
    },
    tempcountc'=3,
    tempcounta'=0,
    tempcountb'=3,
    for tree={
      if={% if the current level exceeds the value of tempcounta
        >OR>{level}{tempcountc}%
      }{}{% then step the count and add the level marker
      if={% if the current level exceeds the value of tempcounta
        >OR>{level}{tempcounta}%
      }{% then step the count and add the level marker
        tempcounta'+=1,
        tempcountb'-=1,
        tikz+/.process={ Rw {tempcountb} {
            \node [anchor=mid east] at (m.east |- .mid) {p=#1};
          }%
        },
      }{}},
    },
  },
[{-1,3},
    [{-1,2}, before computing xy={s'-=50pt}
      [{-1,1}, before computing xy={s'-=15pt}
        [{-1,0} [0, draw=none]]
        [{0,1} [01, draw=none]]
        [{-1,0},color=red  [1, draw=none ]]
      ] 
      [{1,2}, before computing xy={s'-=15pt}
        [{1,0} [10, draw=none]] 
        [{0,2} [102, draw=none]]
        [{1,0},color=red   [12, draw=none] ] 
      ]
      [{-1,1}, before computing xy={s'-=15pt},color=red
        [{0,1},color=red   [2, draw=none] ]
      ]
    ]
    [{2,3}, before computing xy={s'-=48pt}
      [{2,1}, before computing xy={s'-=13pt}
        [{2,0}  [20, draw=none]] 
        [{0,1}  [201, draw=none]]
        [{2,0},color=red  [21, draw=none] ] 
      ] 
      [{1,3}, before computing xy={s'-=13pt}
        [{1,0}  [210, draw=none] ] 
        [{0,3}  [2103, draw=none] ]
        [{1,0},color=red  [213, draw=none] ] 
      ]
      [{2,1}, before computing xy={s'-=13pt},color=red
        [{0,1},color=red [23, draw=none] ]
      ]
  ] 
  [{-1,2}, before computing xy={s'-=53pt},color=red
        [{1,2},color=red, 
         [{0,2},color=red [3, draw=none]]
        ]
  ]
]
\end{forest}
\caption{Parameters $s,t$ in the ternary call tree (simplifying \textcolor{red}{unpebble} branches).}
\label{fig:trees1}
\end{figure*}

\begin{figure}
\begin{forest}
for tree={draw, l sep=15pt},
[{0..8},
    [{0..4},edge label={node[midway,left] {$\times2$}}
      [{0..2},edge label={node[midway,left] {$\times2$}}
        [{0..1},edge label={node[midway,left] {$\times2$}}] 
        [{1..2},edge label={node[midway,right] {}}]
      ] 
      [{2..4},edge label={node[midway,right] {}}
        [{2..3},edge label={node[midway,left] {$\times2$}}] 
        [{3..4},edge label={node[midway,right] {}}]
      ]
    ]
    [{4..8},edge label={node[midway,right] {}}
      [{4..6},edge label={node[midway,left] {$\times2$}}
        [{4..5},edge label={node[midway,left] {$\times2$}}] 
        [{5..6},edge label={node[midway,right] {}}]
      ] 
      [{6..8},edge label={node[midway,right] {}}
        [{6..7},edge label={node[midway,left] {$\times2$}}] 
        [{7..8},edge label={node[midway,right] {}} [{\phantom{a}},draw=none]]
      ]
  ] 
]
\end{forest}
    \caption{Parameters $a,c$ in the ternary call tree, merging pebble/unpebble branches.}
    \label{fig:trees2}
\end{figure}

%\todo{It seems like values in the left figure are uncomputed in wrong order (e.g., 0 before 1), but this is only because the unpebble subtrees are not fully expanded in the figure.}


\begin{lemma}
\label{lem:siar_correct}
SIAR reversibly computes the same values as SIAC (ignoring ancillas).
\end{lemma}

\begin{lemma}\label{lem:siar_complexity}
SIAR uses  $\tsiar \in O(3^{k} \cdot \tsia)$ time and $\ssiar \in O(k\cdot S) = |a_r|$ space.
\end{lemma}

\begin{proof}
The SIAR procedure provides a (uniform, polytime) blueprint for a reversible circuit based on blocks of reversible SIAB circuits: the $S$-sized memory cells $M[-1]$ to $M[k]$ plus the SIAB ancillas $a_b$ make up all the wires of the circuit and the leafs of the call tree of SIAC stipulate how the inputs/outputs of SIAB blocks connect to the wires, i.e, 
\textsf{ M[t]$\xor SIAB_a$(M[s], $a_b$)} (see Example~\ref{ex:1}). 

Since $a_b = \log(n)$, the SIAB ancillas are negligible.
The depth of the ternary call tree is $k$, hence there are $ O(3^k)$ leafs (i.e.~sequentially composed blocks of SIAB circuits).
\end{proof}

\begin{example}\label{ex:1}
Let $k=3$, so that $\zeta=8$. We get the SIAR computation shown in Figure~\ref{fig:trees1} and Figure~\ref{fig:trees2}.

The reversible SIAR circuit based on (reversible) SIA blocks looks as follows (again, the ancillas of SIAB $a_s$ should be interpreted as inputs and outputs):
\begin{center}
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_2$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_3$(M[1], $\vec a_{b}$)}\\
\textsf{ M[2] $\xor SIAB_4$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_3$(M[1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_2$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_5$(M[2], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_6$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_5$(M[2], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_6$(M[1], $\vec a_{b}$)}\\
\textsf{ M[3] $\xor SIAB_7$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_6$(M[1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_5$(M[2], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_6$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_5$(M[2], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_2$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_3$(M[1], $\vec a_{b}$)}\\
\textsf{ M[2] $\xor SIAB_4$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_3$(M[1], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}\\
\textsf{ M[1] $\xor SIAB_2$(M[0], $\vec a_{b}$)}\\
\textsf{ M[0] $\xor SIAB_1$(M[-1], $\vec a_{b}$)}
\end{center}
\end{example}

\begin{theorem}
There is a reversible circuit that computes SIAC for a $w$-biw formula $F$ using only 
 $\tsiar \in O(3^{\log(\zeta)}\cdot w \cdot  d^s \cdot \lolo(n))$ time and
 $\ssiar \in O(\log(\zeta) \cdot (w +\log(n))$ space (wires).
\end{theorem} 

\begin{proof}
By Lemma~\ref{l:sia}, SIAB can be reversibly simulated in
$\tsia \in O(w \cdot d^s \cdot \lolo(n))$  time and $O(w + \log(n))$ wires
(for both inputs+outputs and ancillas). By Lemma~\ref{lem:siar_correct}, SIAR computes SIA, with resource upper bounds following from SIAB's and Lemma~\ref{lem:siar_complexity}.
\end{proof}

Theorem~\ref{t:main} simplifies this theorem. For $w \in o(n/\log(n))$ (which is the case for Lattice SAT), we obtain an algorithm which fits the requirements of the hybrid approach to backtracking algorithms.

\begin{corollary}
\label{coro:SIA-for-hybrid}
There is a $o(n)$-space sub-exponential time reversible implementation of s-SIA for $o(n/\log(n))$-biw formulas.
\end{corollary}

Note that instances of Lattice SAT are Boolean formulas of bounded index width $\sqrt{n} \in o(n/\log(n))$.
